State Complexity of Projection on Languages Recognized by Permutation Automata and Commuting Letters

The projected language of a general deterministic automaton with $n$ states is recognizable by a deterministic automaton with $2^{n-1} + 2^{n-m} - 1$ states, where $m$ denotes the number of states incident to unobservable non-loop transitions, and this bound is best possible. Here, we derive the tight bound $2^{n - \lceil \frac{m}{2} \rceil} - 1$ for permutation automata. For a state-partition automaton with $n$ states (also called automata with the observer property) the projected language is recognizable with $n$ states. Up to now, these, and finite languages projected onto unary languages, were the only classes of automata known to possess this property. We show that this is also true for commutative automata and we find commutative automata that are not state-partition automata.

==> tikz_state_partition.tex <==
\begin{figure}
\label{fig:state_partition}
\centering
\begin{minipage}{0.6\textwidth}
\scalebox{.7}{
\begin{tikzpicture}[>=latex',shorten >=1pt,node distance=1.5cm,on grid,auto,baseline=0]
 \tikzset{every state/.style={minimum size=1pt}}
% \node[state] (1) {};
%  \node[state] (2) [ right of=1] {};
%  \node[state, accepting] (3) [ right of=2] {};
%  \node[state] (2) [below of=1] {};
%  \node[state] (3) [below right of=2] {};
%  \node[state] (4) [below left of=2] {};
%  \node[state] (5) [below left of=4] {};
%  \node[state] (6) [below right of=3] {};
 
%  \path[->] (1) edge node {$a$} (2);
%  \path[->] (2) edge [bend left] node {$a,b$} (3);
%  \path[->] (3) edge [bend left] node {$b$} (2);

 \node [state,initial,accepting] (1) at (90:1.5cm) {$1$};
 \node [state] (2) at (210:1.5cm) {$2$};
 \node [state] (3) at (330:1.5cm) {$3$};
 
 \node [state] (4) at (90:4.5cm) {$4$};
 \node [state] (5) at (207:4.5cm) {$5$};
 \node [state] (6) at (333:4.5cm) {$6$};

  \path[->] (1) edge node {$a$} (2) 
            (2) edge node {$a$} (3)
            (3) edge node {$a$} (1);

  \path[->] (4) edge [left] node {$a$} (5) 
            (5) edge [below] node {$a$} (6)
            (6) edge [right]  node {$a$} (4);
            
 \path[->] (1) edge [bend left=10, pos=.4] node {$b$} (4);
 \path[->] (2) edge [bend left=10, pos=.4] node {$b$} (5);
 \path[->] (3) edge [bend left=10, pos=.4] node {$b$} (6);
 
 \path[->] (4) edge [bend left=10, pos=.6] node {$b$} (1);
 \path[->] (5) edge [bend left=10, pos=.6] node {$b$} (2);
 \path[->] (6) edge [bend left=10, pos=.6] node {$b$} (3);
\end{tikzpicture}}
\end{minipage}%
\begin{minipage}{0.4\textwidth}
 \begin{align*}
  \Orb_{\{b\}}(1) & = \{1,4\} \\
  \Orb_{\{b\}}(2) & = \{2,5\} \\
  \Orb_{\{b\}}(3) & = \{3,6\} \\
  \\
  \Orb_{\{a\}}(1) & = \{1,2,3\} \\ 
  \Orb_{\{a\}}(4) & = \{4,5,6\} \\
  \\
  \pi_{\{a\}}(L(\mathcal A)) & = (aaa)^* \\
  \pi_{\{b\}}(L(\mathcal A)) & = (bb)^* 
 \end{align*}
 %\begin{multline*}
 %    \mathcal T_{\mathcal A} = \{ f : Q \to Q \mid \mbox{$f$ is bijective} \}
 %\end{multline*}
\end{minipage}
\caption{A permutation automaton $\mathcal A = (Q, \{a,b\}, \delta, 1, \{1\})$
 with $Q = \{1,2,3,4,5,6\}$. This is a state-partition automaton
 for $\pi_{\{a\}}$ and $\pi_{\{b\}}$. 
 However, the subgroup $\{ \delta_u \mid u \in \{b\}^* \}$ is not normal
 and the smallest normal subgroup containing it is the whole of $\mathcal T_{\mathcal A} = \{ f : Q \to Q \mid \mbox{$f$ is bijective} \}$.
 Contrary, the subgroup $\{ \delta_u \mid u \in \{a\}^* \}$ is normal.}
\end{figure}
